DyEdgeGAT: Dynamic Edge via Graph Attention for Early Fault Detection in IIoT Systems

In the Industrial Internet of Things (IIoT), condition monitoring sensor signals from complex systems often exhibit nonlinear and stochastic spatial-temporal dynamics under varying conditions. These complex dynamics make fault detection particularly challenging. While previous methods effectively model these dynamics, they often neglect the evolution of relationships between sensor signals. Undetected shifts in these relationships can lead to significant system failures. Furthermore, these methods frequently misidentify novel operating conditions as faults. Addressing these limitations, we propose DyEdgeGAT (Dynamic Edge via Graph Attention), a novel approach for early-stage fault detection in IIoT systems. DyEdgeGAT's primary innovation lies in a novel graph inference scheme for multivariate time series that tracks the evolution of relationships between time series, enabled by dynamic edge construction. Another key innovation of DyEdgeGAT is its ability to incorporate operating condition contexts into node dynamics modeling, enhancing its accuracy and robustness. We rigorously evaluated DyEdgeGAT using both a synthetic dataset, simulating varying levels of fault severity, and a real-world industrial-scale multiphase flow facility benchmark with diverse fault types under varying operating conditions and detection complexities. The results show that DyEdgeGAT significantly outperforms other baseline methods in fault detection, particularly in the early stages with low severity, and exhibits robust performance under novel operating conditions.

==> chaps/00-cov-abs/00-cover.tex <==
% Update your Headers here
\fancyhead[LO]{Temporal Graph Representation Learning for Multivariate Time Series Anomaly Detection}
% \fancyhead[RE]{Firstauthor and Secondauthor} % Firstauthor et al. if more than 2 - must use \documentclass[twoside]{article}


%% Title
\title{Temporal Graph Representation Learning for Multivariate Time Series Anomaly Detection
%%%% Cite as
%%%% Update your official citation here when published 
%\thanks{\textit{\underline{Citation}}: 
%\textbf{Authors. Title. Pages.... DOI:000000/11111.}} 
}

\author{
  Mengjie Zhao, Olga Fink \\
  Intelligent Maintenance and Operations Systems (IMOS) \\
  Swiss Federal Institute of Technology Lausanne (EPFL) \\
  Lausanne, Switerland\\
  \texttt{\{mengjie.zhao, olga.fink\}@epfl.ch} \\
  %% examples of more authors
  % \And
  %Author3 \\
  %Affiliation \\
  %Univ \\
  %City\\
  %\texttt{email@email} \\
  %% \AND
  %% Coauthor \\
  %% Affiliation \\
  %% Address \\
  %% \texttt{email} \\
  %% \And
  %% Coauthor \\
  %% Affiliation \\
  %% Address \\
  %% \texttt{email} \\
  %% \And
  %% Coauthor \\
  %% Affiliation \\
  %% Address \\
  %% \texttt{email} \\
}

==> chaps/bk/02-3-tgnn_bk.tex <==
%\subsection{Modelling Inter-dependencies and Dynamics with Graphs}
Within the discrete-time framework, temporal graphs are represented by a series of static graph snapshots, sequentially arranged over time. This approach incorporates two common methodologies: \textit{graph-then-time} and \textit{time-and-graph}. 
Conversely, the continuous-time representation, often termed \textit{time-then-graph}, presents temporal dynamics within a static graph structure. Gao \textit{et al.}~\cite{gao2022equivalence} provide a more thorough definition of these frameworks.
% examples
Existing work primarily focuses on modeling temporal graphs for MTS using a discrete graph representation and aligns with the \textit{time-and-graph} architecture.
Many spatial-temporal GNNs belong to this category, including 
Diffusion Convolutional Recurrent Neural Network (DCRNN)~\cite{li2017diffusion} that utilizes SpectralGCN to capture spatial dependency and then GRU to capture the temporal dependency, and Multivariate Time-series Anomaly Detection via Graph Attention Network (MTADGAT)~\cite{zhao2020mtadgat}, which constructs feature and temporal graphs to capture inter-dependencies between time series, followed by a GRU to extract dynamics.
% limitation
Despite the predominance of the discrete-time representation, Gao \textit{et al.}~\cite{gao2022equivalence} have demonstrated in their recent paper that the \textit{time-then-graph} representation is strictly more representative than the other two representations, making it more appropriate for anomaly detection in MTS.
However, implementing this representation remains a challenge, especially in the context of MTS where the graph must be inferred.
This framework has been predominantly applied to graph-structured networks such as evolving social networks, examples of which include Temporal Graph Network (TGN)~\cite{rossi2020tgn} and Temporal Graph Attention Networks (TGAT)~\cite{xu2020tgat}, where the graph topology is provided implicitly. 
Currently, there is no existing work on jointly constructing a graph from MTS and applying continuous graph representation to it.
We believe this approach would offer greater expressiveness compared to the discrete graph representation of MTS, thus enhancing its effectiveness in detecting abnormal changes in functional relations within MTS.

% Temporal Graph Neural Networks (TGNNs) are applied to effectively extract the temporal and inter-dependencies from the MTS data.
% in graphs~\cite{zaki2016comprehensive}, making them particularly relevant for MTS anomaly detection. 

%\subsubsection{Continuous time representation in GNNs}
%In the continuous-time representation, all past node and edge attributes are integrated into a single static graph. This representation captures the entire history of temporal dynamics. An encoder function is used to encode node attributes and another encoder function is used to encode edge attributes. The encoded representations are then passed through a GNN to model the interactions and dependencies in the continuous-time graph.
% time-then-graph
%An example of the \textit{time-then-graph} framework is TGAT~\cite{xu2020tgat}, which memorizes the edges of past snapshots to create a static heterogeneous graph, used to extract the final temporal graph representations. TGN~\cite{rossi2020tgn} extends this framework by incorporating a memory module. Studies by Gao \textit{at al.}~\cite{gao2022equivalence} have demonstrated the superior expressiveness of GRU-GCN over GCN-GRU in continuous-time representation.




%\subsubsection{Discrete time representation in GNNs}
%In the discrete-time representation, a temporal graph consists of a sequence of static graph snapshots over multiple time steps. Each snapshot is processed by a static GNN to encode the graph structure at that time step. To model the temporal dynamics, an aggregation function, such as an RNN, is used to aggregate the graph encodings across all snapshots.
% examples
%Notable approaches in this framework include EvolveGCN~\cite{pareja2020evolvegcn}, which learns temporal dynamics through GCN parameters and passes them as recurrent states, and Dynamic Self Attention (DySAT)~\cite{sankar2020dysat}, which introduced the first discrete TGNN based solely on attention. 
%ROLAND~\cite{you2022roland} extends static GNNs to dynamic settings by updating node embeddings based on newly observed nodes and edges using a GRU update module.
% time-and-graph
%The \textit{time-and-graph} framework extends the \textit{graph-then-time} approach by incorporating an additional GNN layer to encode historical snapshot representations.
% examples
% GCRN-M2~\cite{seo2018structured} which combine SpectralGCN~\cite{defferrard2016convolutional} with LSTM, DCRNN~\cite{li2017diffusion} which uses a combination of SpectralGCN and GRU. 
%Many spatial-temporal GNNs belong to this category, auch as T-GCN~\cite{zhao2019tgcn}, STGCN~\cite{yu2018spatio}, MTGNN\cite{wu2020mtgnn} and GTS~\cite{shang2021gts}.

%In the discrete-time representation, two common frameworks are employed: \textit{graph-then-time} and \textit{time-and-graph}. 
%In the discrete graph representation, a temporal graph consists of a sequence of static graph snapshots over multiple time steps.
%The continuous-time representation is also referred to as \textit{time-then-graph}, capturing temporal dynamics within a static graph structure. 
%For a more comprehensive definition, readers can refer to the work of Gao \textit{et al.}~\cite{gao2022equivalence}.

%Temporal or dynamic graphs derived from MTS data can effectively incorporate the inherent inter-dependencies and dynamics present in the data.
%There are two common frameworks to represent temporal graphs: \textit{discrete-time} and \textit{continuous-time} graph representations~\cite{zaki2016comprehensive}. 

==> chaps/bk/02-3-time-then-graph_bk.tex <==
\subsection{Dynamic Interaction Modeling }
\label{sec:method_graph_repr}
\revtextrewrite{
%To address the complexity of temporal and spatial dynamics in IIoT systems, DyEdgeGAT employs the \textit{time-then-graph} framework based on the aggregated temporal graph representation. 
%The \textit{time-then-graph} framework in DyEdgeGAT, as the name suggests, sequentially extracts temporal patterns using a sequence model and captures spatio-temporal relationships using GNNs. These two steps are elaborated in detail below.

\textbf{First time}. During the temporal dynamics extraction phase, Gated Recurrent Units (GRUs) followed by Layer Normalization (LN) and activation functions are utilized for both, nodes and edges to model dynamics over the time window $[t_w, t]$ of length $W$. The dynamics are encoded as:
\begin{align}
\mathbf{H}^{node} &= \text{GRU}^{\text{node}}(\mathbf{X}^{t_w:t}, \mathbf{U}^{t_w:t}), \quad \forall i \in \mathcal{V}, \label{eq:node_dyn}\\
\mathbf{H}^{edge} &= \text{GRU}^{\text{edge}}(\mathbf{A}^{t_w:t}), \quad \forall (i,j) \in \mathcal{E}, \label{eq:edge_dyn}
\end{align}
where $\mathbf{H}^{\text{node}} \in \mathbb{R}^{N\times d_n}$ and $\mathbf{H}^{\text{edge}} \in \mathbb{R}^{N \times N }$ denote the latent dynamics representations of nodes and edges, respectively, with $d_n$ representing the hidden node feature dimensions. 
Here, $\mathcal{V}$ is the set of nodes, and $\mathcal{E}$ is the set of edges. 
In Eq.~\ref{eq:node_dyn}, the matrix $\mathbf{X}^{t_w:t} \in \mathbb{R}^{N \times W}$ represents the sliding window of system-dependent signals, while $\mathbf{U}^{t_w:t} \in \mathbb{R}^{N_u \times W}$ represents system-independent signals, capturing external factors or control variables.
These system-independent signals $\mathbf{U}^{t_w:t}$ reflect the operating conditions of the system and should be treated separately from the dynamics of the system-dependent measurements $\mathbf{X}^{t_w:t}$. In Sec.~\ref{sec:method_oc_recon}, we will elaborate in more detail on how the context of operating conditions is augmented in Eq.\ref{eq:node_dyn}.
In Eq.~\ref{eq:edge_dyn}, $\mathbf{A}^{t_w:t}\in \mathbb{R}^{N \times N \times W}$  represents a sequence of aggregated edge weights over \( [t_w, t] \), which differing from the conventional spatial-temporal graph approach where $\mathbf{A}$ is assumed to be static for each input $\mathbf{X}^{t_w:t}$. Therefore, it is necessary to construct dynamic edges to capture the evolving interactions, and further details on this construction will be provided in Sec.~\ref{sec:method_graph_constr}.

\textbf{Then graph}. Upon obtaining the temporal features, the graph processing phase leverages GNNs followed by Batch Normalization (BN) layers to integrate the node and edge dynamics into an aggregated graph representation:
\begin{align}
\mathbf{Z} &= \text{GNN}^L(\mathbf{H}^{\text{node}}, \mathbf{H}^{\text{edge}}), \label{eq:gnn}
\end{align}
where $\mathbf{Z} \in \mathbb{R}^{N\times d_z}$ denotes the output representation of the nodes after $L$ layers of GNN processing, with $d_z$ being the dimensionality of the output space, and $\mathbf{Z}^0$ initialized with  $\mathbf{H}^{\text{node}}$.
}
\revtext{
The GNN layer in Eq. \ref{eq:gnn} follows the Message Passing Neural Network (MPNN) schema~\cite{gilmer2017neural}. In this framework, the $l$-th layer of a GNN consists of a step of message passing and update:
\begin{align}
    \mathbf{m}^{(l)}_i &= \sum_{j \in \mathcal{N}_i} \text{MSG}^{(l)} (\mathbf{z}^{(l-1)}_i, \mathbf{z}^{(l-1)}_j, \tilde{{a}}_{ij}), \\
    \mathbf{z}^{(l)}_i &= \text{UPDATE}^{(l)} (\mathbf{z}^{(l-1)}_i, \mathbf{m}^{(l)}_i).
\end{align}
Here, $\mathcal{N}_i$ denotes the neighborhood of node $i$, $\mathbf{m}^{(l)}_i$ is the message accumulated at node $i$ in layer $l$, and ${\tilde{{a}}}_{jk}$ represents the edge weights between nodes $j$ and $k$ of the aggregated temporal graph. The functions $\text{MSG}$ and $\text{UPDATE}$ are learnable transformations specific to the GNN architecture, which aggregate neighbor information and update the node representation, respectively.
Specifically, we employ Graph Isomorphism Network (GIN)~\cite{xu2018gin} as the GNN module and employ Batch Normalization (BN) between its layers. An overview of the DyEdgeGAT framework can be found in Fig.\ref{fig:dyedgegat_overview}.
}

%The \textit{time-then-graph} framework in DyEdgeGAT extracts temporal patterns via sequence models and spatio-temporal relationships through  GNNs. As the name suggests, it operates in two consecutive phases: the extraction of temporal dynamics followed by graph processing. Through continuous temporal representation, it can better capture the evolution of the relationships between sensor signals.


% Another important observation relates to $\mathbf{A}^{t_w:t}$ in Eq.~\ref{eq:edge_dyn}. Traditional GNN-based methods consider $\mathbf{A}$ as static for the sliding MTS sequence (or for the entire time series). However, in order to extract edge dynamics, it is necessary to construct dynamic edges. We will elaborate on this aspect in Sec.~\ref{sec:method_graph_constr}.



% We formally define a graph as $\mathcal{G}=(\mathcal{V}, \mathcal{E})$, where $\mathcal{V}=\{v_i\}$ is the set of nodes and $\mathcal{E}=\{e_{ij}\}$ is the set of edges.
%We represent a temporal graph over a sliding window of $w$ time steps as a single, aggregated static graph $\mathcal{G}=(\mathbf{X}^{t_w:t}, \mathbf{A}^{t_w: t})$, where $\mathbf{X}^{t_w:t}=[\mathbf{X}^{t_w},\cdots,\mathbf{X}^t]  \in \R^{|\mathcal{V}|\times W}$ represents the node attributes, and $\mathbf{A}^{t_w:t}=[\mathbf{A}^{t_w},\cdots,\mathbf{A}^t] \in \R^{|\mathcal{V}|\times|\mathcal{V}|\times W} $ represents the edge attributes. These attributes integrate all past node and edge information, as defined in~\cite{gao2022equivalence}.

%is to first represent the evolving relationships of node and edge attributes as sequences and subsequently embed these sequences in a static graph using a GNN.

%Here, $H^{node}$ and $H^{edge}$ represent the evolving node and edge representations, respectively. $E$ denotes the set of all possible edges in an aggregated form, and $Z$ yields the final temporal graph representation encompassing all nodes.


%A temporal encoder $f$ is used to extract the dynamics of node and edge attributes. The resulting node and edge representations are utilized as the node and edge attributes in a new (static) graph, which is subsequently encoded by a Graph Neural Network (GNN). Following the notation of Gao \textit{et al.}~\cite{gao2022equivalence}, we define the aggregated temporal graph as follows:
%\begin{align}
%    \mathbf{H}^{node} &= f^{node}(\mathbf{X}^{t_w:t}, \mathbf{U}^{t_w:t}), \quad \forall i \in \mathcal{V}, \label{eq:node_dyn}\\ 
%    \mathbf{H}^{edge} &= f^{edge}(\mathbf{A}^{t_w:t}), \quad \forall (i,j) \in \mathcal{E}, \label{eq:edge_dyn}\\
%    \mathbf{Z} &= \text{GNN}^L(\mathbf{H}^{node}, \mathbf{H}^{edge})\label{eq:gnn}.
%\end{align}
%Here, $\mathbf{H}^{node} \revtext{\in \R^{|\mathcal{V}|\times d_n}}$ and $\mathbf{H}^{edge} \revtext{\in \R^{|\mathcal{E}|\times d_e}}$ represent the dynamics of nodes and edges, respectively. $\mathcal{E}$ denotes the set of all possible edges in an aggregated form, and $\mathbf{Z}$ represents the final temporal graph representation of all nodes. $L$ corresponds to the number of GNN layers. For the node encoder $f^{node}$ and edge encoder $f^{edge}$, we use separate GRU models, followed by a Layer Norm (LN) and an activation function to extract dynamics. The GNN model is then employed to learn the graph representation, utilizing the Graph Isomorphism Network (GIN)~\cite{xu2018gin} as the graph module and incorporating Batch Normalization (BN) between the GNN layers.

%Here, \(\mathbf{H}^{node} \in \R^{|\mathcal{V}|\times d_n}\) and \(\mathbf{H}^{edge} \in \R^{|\mathcal{E}|\times d_e}\) depict the dynamics of nodes and edges. \(\mathcal{E}\) signifies all potential edges in aggregated form, with \(\mathbf{Z}\) as the overall temporal graph representation. For node and edge encoders, separate GRU models enhanced with Layer Norm (LN) and activation functions are employed. The GNN employs the Graph Isomorphism Network (GIN) with Batch Normalization (BN) interleaved between its layers.


%Note that in the original formulation, $f^{node}$ in Eq.~\ref{eq:node_dyn} is a function of only $\mathbf{X}^{t_w:t}$. However, we argue that the control variables provide valuable information about the operating conditions of the system and should be treated separately from the dynamics of the measurements. Therefore, they are modeled differently. In Sec.~\ref{sec:method_oc_recon}, we provide a detailed explanation of how we include the control variables in the node encoding function to capture the context of the operating conditions.

==> chaps/bk/03-0-preliminaries_bk.tex <==
\section{Preliminaries}
%\revtextrewrite{
%In this paper, we utilize bold uppercase letters (e.g., $\mathbf{X}$), bold lowercase letters (e.g., $\mathbf{x}$), and calligraphic letters (e.g., $\mathcal{V}$) to denote matrices, vectors, and sets, respectively.

%\subsection{Problem Statement}
% state how MTS is defined in a sensor network
%In an IIoT sensor network, $N$ system-dependent measurement signals at any time $t$ are represented as $\mathbf{x}^{t} = [x_{1}^{t}, \cdots, x_{N}^{t}] \in \R^{N}$, where $x_{i}^{t}$ represents the $i^{th}$ sensor's time series at time $t$. 
%By employing a sliding window approach of length $W$, we construct samples as:
%$\mathbf{X}^{t_w:t} = [\mathbf{x}^{t_w}, \cdots, \mathbf{x}^{t-1}, \mathbf{x}^{t}] \in \R^{N \times W}$, where $t_w = t - W + 1 > 0$. 
%Similarly, system independent variables (control variables and external variables) are denoted $\mathbf{U}^{t_w:t} \in \R^{N_u \times W}$.
%The proposed method, DyEdgeGAT, employs a reconstruction model $f_\theta$ for unsupervised MTS fault and anomaly detection.
%The model generates an output $\mathbf{\hat{X}}^{t_w:t} = f_\theta(\mathbf{X}^{t_w:t}, \mathbf{U}^{t_w:t})$ for each $N_{train}$ healthy samples, aiming to minimize the reconstruction discrepancy $||\mathbf{\hat{X}}^{t_w:t} - \mathbf{X}^{t_w:t}||$.
%At test time, the model outputs $\mathbf{y} \in \R^{N_{test}}$ for all $N_{test}$ samples based on the reconstruction discrepancy, where each element $\mathbf{y}_i \in \{0, 1\}$ indicates fault or anomaly.
%}

\subsection{Multivariate Time Series as Temporal Graph}
\label{sec:prelim_graph_repr}
\revtext{
%Given the significance of analyzing the evolving relationships in the IIoT systems, it becomes important to understand the underlying structure and relationships of these MTS data. 
Temporal graphs, also referred to as spatial-temporal or dynamic graphs (with no distinction among these terms in our context), present a promising data format for MTS analysis in the IIoT context. 
%These graph structures effectively capture the temporal dynamics of MTS data, allowing downstream analysis of the relationships within the network over time~\cite{jin2023survey}. 
There are primarily two \textit{equivalent} approaches to represent these temporal graphs following the definition by Gao et al.~\cite{gao2022equivalence}.



\textbf{Discrete-Time Dynamic Graph}. 
Conceptualized  as a sequence of attributed graphs at discrete time steps, a discrete-time dynamic graph within  a time window from $t_w$ to $t$ can be represented as:
\[\mathcal{G} = \{\mathcal{G}^{t_w}, \ldots, \mathcal{G}^t\}.\]
At each time instance \( t \), we define \( \mathcal{G}^t = (\mathbf{A}^t, \mathbf{x}^t) \) as the attributed graph, where $\mathbf{A}^t \in \R^{N \times N}$ represents  the adjacency matrix and $\mathbf{x}^t \in \R^{N}$ denotes the feature matrix.

\textbf{Aggregated Temporal Graph}.
An alternative representation, as proposed by Gao et al.~\cite{gao2022equivalence}, is the aggregated temporal graph, where the graph is treated as a static graph  aggregating information from all time steps:
\[ \mathcal{G} = (\mathbf{X}^{t_w:t}, \mathbf{A}^{t_w: t}),  \]
Here, $\mathbf{X}^{t_w:t}=[\mathbf{x}^{t_w},\cdots,\mathbf{x}^t]  \in \R^{N\times W}$ represents all node attributes aggregated within the time window, while $\mathbf{A}^{t_w:t}=[\mathbf{A}^{t_w},\cdots,\mathbf{A}^t] \in \R^{N\times N \times W}$ represents aggregated edge attributes as sequences of standalone attributes, with zeros for absent attributes.
}

% In case of IIoT with heterogenous sensors, each sensor is treated as a separate sensor, so $D=1$.


%A temporal graph observed over a sliding window of $w$ time steps can be represented as a sequence of static graph snapshots. 

%Formally, it is defined as: $ \{ (\mathbf{X}^{t}, \mathbf{A}^{t}) \}^T_{t=t_w} $

%\textbf{Attributed Graph}.
%An attributed graph is a static graph that associates each node with a set of attributes, representing node features. Formally, an attributed graph is defined as $\mathcal{G}=(\mathbf{X}, \mathbf{A})$, 
%where $\mathbf{X} \in \mathbb{R}^{N \times D}$ is the node attribute matrix, where each row represents the attributes of a node and $D$ denotes the dimensionality of the node attributes.
%And \( \mathbf{A} \in \mathbb{R}^{N \times N} \) is the adjacency matrix, indicating the presence (or weight) of edges between nodes. An entry \( A_{ij} \) is non-zero if an edge \( e_{ij} \) exists between nodes \( v_i \) and \( v_j \).

%In light of the attributed graphs, a temporal graph can be described as a series of attributed graphs, which effectively represent (multivariate) time series data in conjunction with evolving structural information over time.

%\textbf{Discrete-Time Dynamic Graph}. A discrete-time dynamic graph can be visualized through a series of attributed graphs at various discrete time steps. This graph can be represented as \( \mathcal{G} = \{\mathcal{G}^1, \mathcal{G}^2, \ldots, \mathcal{G}^T\} \), where for each time point \( t \), \( \mathcal{G}^t = (\mathbf{A}^t, \mathbf{X}^t) \) signifies the attributed graph. Here, \( \mathbf{A}^t \) in \( \R^{N \times N} \) and \( \mathbf{X}^t \) in \( \R^{N \times D} \) are the adjacency and feature matrices respectively. The adjacency matrix \( \mathbf{A}^t \) might transform as time progresses or could remain static, subject to the particular configurations in place. When we're generalizing time series data into this format, we express \( \mathbf{X}^t \) as a column vector \( \mathbf{x}^t \) with its elements from \( \mathbb{R}^N \).


%When time series data is generalized into this format, \( \mathbf{X}^t \) is expressed as a column vector \( \mathbf{x}^t \) with elements from \( \mathbb{R}^N \).##


%A discrete-time dynamic graph can be visualized through a series of attributed graphs at various discrete time steps. 
%Given sliding window of $W$ time steps from $t_w$ to $t$, 
%This graph is represented as \( \mathcal{G} = \{\mathcal{G}^{t_w}, \ldots, \mathcal{G}^t\} \). For each time point \( t \), \( \mathcal{G}^t = (\mathbf{A}^t, \mathbf{x}^t) \) is defined as the attributed graph. Here, \( \mathbf{A}^t \) \in \( \R^{N \times N} \) and \( \mathbf{x}^t \) \in \( \R^{N} \) are known as the adjacency and feature matrices, respectively. The adjacency matrix \( \mathbf{A}^t \) may be transformed as time progresses or remain static, depending on the particular configurations chosen. 


==> chaps/bk/03-framework_bk.tex <==
\section{Proposed Framework}

\subsection{Problem Statement}
% statement of the task (should I mention in addition change of relationship in time?)
Multivariate time-series anomaly detection aims to detect anomalies at the entity level. This is especially challenging due to the complex dependencies and temporal dynamics exhibited by multivariate time-series data.
% state how MTS is defined in a sensor network
Sensor measurements can be modeled as a sequence of $N$ Multivariate Time Series (MTS) at a time $\mathbf{X}^{t_w:t} = \lbrack\mathbf{x}_{1}^{t_w:t},\cdots \mathbf{x}_{N}^{t_w:t}\rbrack\ \in \R^{N\times W}$, where $t$ is the current time step and $W=t-t_w+1>0$ is the length of the observation window.
Similarly, control variables can be modelled as: $\mathbf{U}^{t_w:t} = \lbrack\mathbf{u}_{1}^{t_w:t},\cdots \mathbf{u}_{N}^{t_w:t}\rbrack\ \in \R^{N_u\times W}$
% TODO: introduce sliding window
% anomaly detection task
The task of multivariate  time-series  anomaly  detection  is  to  produce  an output vector $\mathbf{y} \in \R^n$, where $\mathbf{y}_i \in \{0,1\}$ denotes whether the $i$-th timestamp is an anomaly. The mathematical notations are presented in Table~\ref{tab:notations}.
\input{tabs/notations}

\subsection{Overview}
Our proposed method, \textit{\revtext{TimeGAT}} (Dynamic Graph Attention for Anomaly Detection), is specifically designed to address the dynamic nature of multivariate time series by modeling relationship changes over time. By effectively capturing the complex inter-feature correlations and temporal dependencies, \revtext{TimeGAT} is able to robustly detect anomalies in multivariate time series data. 
The key mechanisms that enable this are a temporal graph representation learning scheme and an operating condition-aware reconstruction mechanism. 
% TODO: add bullet point summary
In the following subsections, we elaborate on the core components of the \revtext{TimeGAT}.

\subsection{Multivariate Time Series as a Temporal Graph}
We first introduce how we present the Multivariate Time Series (MTS) in the form of a Continuous Time Temporal Graph (CTTG). We represent a temporal graph over $T$ time steps as a single, aggregated static graph $G(\mathbf{X}_{t\leq T}, \mathbf{A}_{t\leq T})$, where $\mathbf{X}_{t\leq T}$ is the raw signal input, and $\mathbf{A}_{t\leq T}$ is the learned dynamic edge.

\subsection{\revtext{TimeGAT} Temporal Graph Construction}
This section explains how $\mathbf{X}_{t\leq T}$ and $\mathbf{A}_{t\leq T}$ are formed and learned.

\subsubsection{Raw Signal Input}
The raw signal input $\mathbf{X}_{t\leq T} = [\mathbf{X}_1,\cdots,\mathbf{X}_T]$ represents the original multivariate time series data integrated over all past time steps.

\subsubsection{Dynamic Edge Learning}
The dynamic edge $\mathbf{A}_{t\leq T} = [\mathbf{A}_1,\cdots,\mathbf{A}_T]$ is learned using an attention-based approach. We employ a sliding window method to capture the temporal dependencies within the multivariate time-series data. Our graph attention mechanism is built upon the GATv2~\cite{brody2022gatv2} algorithm, which enhances the original Graph Attention Networks (GAT) by overcoming its static attention limitation.

\subsection{Temporal Graph Representation Learning}
After forming the raw signal input and dynamic edge, we use a temporal encoder $f$ to extract the dynamics of node and edge attributes. The resulting node and edge representations become the node and edge attributes in a new (static) graph, which is then encoded by a GNN.

\begin{align}
    \mathbf{H}^{node} &= f^{node}(\mathbf{X}_{t\leq T}), \forall i \in \mathcal{V} \\
    \mathbf{H}^{edge} &= f^{edge}(\mathbf{A}_{t\leq T}), \forall (i,j) \in \mathcal{E} \\
    \mathbf{Z} &= \text{GNN}(H^{node}, H^{edge})
\end{align}

where $H^{node}$ and $H^{edge}$ are the representations of node and edge evolutions, $\mathcal{E}$ is the set of all possible edges in aggregated form, and $Z$ is the final temporal graph representation of all nodes. We use a GRU to extract both edge and node dynamics ($f^{node}=\text{GRU}^{node}$ and $f^{edge}=\text{GRU}^{edge}$) and GCN ($GNN=GCN$) to learn the graph representation. The learned feature attention in this continuous time representation is dynamic, unlike static attention in discrete representations.


%In our case, each $\mathbf{x}_i$ is associated with a graph node $v_i$.

%We define an attributed graph as $\mathcal{G}=(\mathbf{X}, \mathbf{A})$, where $\mathbf{X} \in \R^{N\times w}$ are the node attributes and $\mathbf{A} \in \R^{N\times N}$ are the edge attributes.

%A graph structure can be created by representing each time series as a node in the graph and using edges to represent the interactions between the time series. In general, 

%A temporal graph is created by representing each time series as a node in the graph, and the edges represent the interactions between the time series. The temporal graph over $T$ time steps is represented as a single aggregated static graph $G(\mathbf{X}_{t\leq T}, \mathbf{A}_{t\leq T})$, where $\mathbf{X}_{t\leq T}$ and $\mathbf{A}_{t\leq T}$ integrate all past node and edge attributes~\cite{gao2022equivalence}. The temporal encoder extracts the dynamics of node and edge attributes, and the resulting representations become the attributes of the new (static) graph. The GNN is then applied to this graph to learn the representations.

%\subsection{Time-then-graph Representation}
% graph learning task
%A graph structure can be created by representing each time series as a node in the graph and using edges to represent the interactions between the time series. In general, a graph is defined $\mathcal{G}=(\mathcal{V}, \mathcal{E})$ as a set of nodes $\mathcal{V}=\{v_i\}$ and edges $\mathcal{E}=\{e_{ij}\}$. In our case, each $\mathbf{x}_i$ is associated with a graph node $v_i$.
%We define an attributed graph as $\mathcal{G}=(\mathbf{X}, \mathbf{A})$, where $\mathbf{X} \in \R^{N\times w}$ are the node attributes and $\mathbf{A} \in \R^{N\times N}$ are the edge attributes.

% Time then graph
%We represent a temporal graph over $T$ time steps as a single, aggregated static graph $G(\mathbf{X}_{t\leq T}, \mathbf{A}_{t\leq T})$, where $\mathbf{X}_{t\leq T}=[\mathbf{X}_1,\cdots,\mathbf{X}_T]$, $\mathbf{A}_{t\leq T}=[\mathbf{A}_1,\cdots,\mathbf{A}_T]$ integrate all past node and edge attributes~\cite{gao2022equivalence}. 

%A temporal encoder $f$ extracts the dynamics of node and edge attributes, and the resulting node and edge representations become the node and edge attributes in a new (static) graph, which is then encoded by a GNN. 

%The two steps of a continuous TGNN as introduced in~\cite{gao2022equivalence} are: 
%\begin{align}
%    \mathbf{H}^{node} &= f^{node}(\mathbf{X}_{t\leq T}), \forall i \in \mathcal{V} \\
%    \mathbf{H}^{edge} &= f^{edge}(\mathbf{A}_{t\leq T}), \forall (i,j) \in \mathcal{E} \\
%    \mathbf{Z} &= \text{GNN}(H^{node}, H^{edge})
%\end{align}
%where Hnode and Hedge are the representations of node and edge evolutions, E is the set of all possible edges in aggregated form and Z is final temporal graph representation of all nodes. We use GRU to extract both edge and node dynamics ($f^{node}=\text{GRU}^{node}$ and $f^{edge}=\text{GRU}^{edge}$) and GCN to learn the graph representation. The learned feature attention in this continuous time representation is dynamic, unlike static attention in discrete representations.



To capture the temporal dynamics and dependencies in multivariate time series data, \revtext{TimeGAT} utilizes the \textit{time-then-graph} representation. 
Formally, we define a graph as $\mathcal{G}=(\mathcal{V}, \mathcal{E})$, where $\mathcal{V}=\{v_i\}$ is the set of nodes and $\mathcal{E}=\{e_{ij}\}$ is the set of edges.

We represent a temporal graph over a sliding window of $w$ time steps as a single, aggregated static graph $\mathcal{G}=(\mathbf{X}^{t_w:t}, \mathbf{A}^{t_w: t})$, where $\mathbf{X}^{t_w:t}=[\mathbf{X}^{t_w},\cdots,\mathbf{X}^t]  \in \R^{|\mathcal{V}|\times W}$ represents the node attributes, and $\mathbf{A}^{t_w:t}=[\mathbf{A}^{t_w},\cdots,\mathbf{A}^t] \in \R^{|\mathcal{V}|\times|\mathcal{V}|\times W} $ represents the edge attributes. These attributes integrate all past node and edge information, as defined in~\cite{gao2022equivalence}.

A temporal encoder $f$ is used to extract the dynamics of node and edge attributes. The resulting node and edge representations become the node and edge attributes in a new (static) graph, which is then encoded by a Graph Neural Network (GNN). We adopt the notation from Gao \textit{et al.}~\cite{gao2022equivalence} and define the aggregated temporal graph as follows:
\begin{align}
    \mathbf{H}^{node} &= f^{node}(\mathbf{X}^{t_w:t}, \mathbf{U}^{t_w:t}), &\forall i \in \mathcal{V}, \label{eq:node_dyn}\\ 
    \mathbf{H}^{edge} &= f^{edge}(\mathbf{A}^{t_w:t}), &\forall (i,j) \in \mathcal{E}, \label{eq:edge_dyn}\\
    \mathbf{Z} &= \text{GNN}(\mathbf{H}^{node}, \mathbf{H}^{edge}).
\end{align}
Here, $\mathbf{H}^{node}$ and $\mathbf{H}^{edge}$ represent the node and edge dynamics, respectively. $\mathcal{E}$ is the set of all possible edges in aggregated form, and $\mathbf{Z}$ is the final temporal graph representation of all nodes. We use the two seperate GRU models to extract edge and node dynamics, and employ the GCN model to learn the graph representation. The learned feature attention in this continuous time representation is dynamic, unlike the static attention in discrete representations.

Note that in the original formulation, $f^{node}$ in Eq.~\ref{eq:node_dyn} is a function of only $\mathbf{X}^{t_w:t}$. However, we argue that the control variables provide information about the operating condition of the system and are different from the dynamics of the measurements. Therefore, they should be modeled differently.

==> chaps/bk/04-2-baseline-bk.tex <==
\subsection{Baselines}
% TODO: link to the result section, which categorizes methods into three groups
For a comprehensive evaluation of our proposed method, we compare its performance to a range of state-of-the-art novel anomaly detection methods, 
which can be classified into two primary categories: prediction-based and reconstruction-based methods. 

Specifically, we group the methods with their abilities to model MTS.

Our objective is to examine the effectiveness of each of these techniques in identifying anomalies, specifically those that arise from changing relations within dynamic systems. This evaluation requires an understanding of the interdependencies between signals as they evolve over time.

\input{tabs/baselines_tab}

%\begin{itemize}
\textbf{FNN}: The Feed-forward Neural Network-based anomaly detection method establishes a mapping between control variables and measurement variables, providing a basic model of the system's internal relationships. It should be noted that this approach does not incorporate temporal information, and may potentially miss dynamic anomalies.

\textbf{AE}~\cite{aggarwaloutlier}: Autoencoders, similar to FNN, attempt to capture interdependencies within the data by reconstructing input data and detecting anomalies based on higher reconstruction errors. Similarly to FNN, they do not factor in temporal information.

\textbf{LSTM}~\cite{malhotra2015lstmad}: Long Short-Term Memory Networks (LSTM) capture temporal patterns within the data and identify anomalies through deviations from predicted values. While they effectively incorporate temporal information, LSTMs do not distinguish between the control variables and the measurement variables and may not model complex interdependencies between the sensors as effectively.

\textbf{ENCDEC-AD}~\cite{malhotra2016encdecad}: The LSTM-based encoder-decoder architecture seeks to capture both temporal and inter-dependencies, providing a more comprehensive model of system behavior. It takes sequences of control and measurement variables as input and outputs control and measurement variables

\textbf{MTADGAT}\cite{zhao2020mtadgat}: Multivariate Time-series Anomaly Detection via Graph  Attention Network combines feature-oriented GAT\cite{velivckovic2017gat} and time-oriented GAT to handle spatial dependencies and temporal dependencies simultaneously. By performing forecasting and reconstruction concurrently, MTADGAT can model complex relationships and dynamics.
It does not distinguish control from measurement variables and treats them as identical types of nodes in the graph construction.

\textbf{GDN}~\cite{deng2021gdn}: Graph Deviation Network (GDN) has demonstrated to be particularly good in modeling intricate relationships in the data. It constructs a static graph based on the cosine similarity of the training batch data, uses sensor embedding to distinguish sensor types, and employs an attention mechanism for forecasting. Like MTADGAT, control variables are included in the learned graph as measurement variables.

%\end{itemize}
These baseline methods were carefully selected to test their ability to detect different types of anomalies, each with unique strengths in detecting different types of anomalies - those where temporal relationships are crucial and those primarily driven by inter-dependencies between signals. Consequently, they provide a comprehensive comparison for assessing the performance of our proposed method, \revtext{TimeGAT}.
Hyperparameter tuning for these baseline models was performed separately for both the synthetic and the industrial (Pronto) datasets to ensure optimal performance in each case study. 
It is important to note that, for MTADGAT, we opted for a modification of the original implementation, adopting the more expressive GATv2~\cite{brody2022gatv2} instead of the original GAT. 
The selection of the final model architectures was based on their Mean Absolute Error (MAE) on the validation sets. Detailed information about the hyperparameters used for each model can be found in Appendix~\ref{sec:app_hyperparameters}.

% anomaly score evaluations
For all the baselines, we employ the same anomaly score function introduced by GDN~\cite{deng2021gdn}. To account for the varying characteristics of the residuals of different sensors and prevent any single sensor from dominating the anomaly detection process, the anomaly score $s_i^t$ of a signal $i$ at time $t$ is a normalized residual $r_i^t$, defined as:
\begin{equation}
s_i^t=  \frac{ |r_i^t - \Tilde{\mu_i}|}{\Tilde{\sigma_i}}
\end{equation}
where $\Tilde{\mu_i}$ and $\Tilde{\sigma_i}$ are the median and inter-quartile range (IQR) of the validation set error. 
Please note that in their case study, the author of the GDN paper \cite{deng2021gdn} utilizes a max aggregator over all nodes, which is suitable for datasets primarily comprising point anomalies. 
However, in our study where functional relation changes may affect multiple signals, we employ a mean aggregator to capture the collective impact on the signals.
Additionally, for ENCDEC-AD and MTAD-GAT, we also average the anomaly score over time.

==> chaps/bk/05-2-2-pronto-fault-types-duplicated.tex <==
%\subsubsection{Fault Types Specific Performance on Pronto Dataset}
\label{sec:pronto-fault}

\begin{figure}[htbp]
\centering
\includegraphics[width=.9\linewidth]{figs/pronto/pronto_auc.pdf}
\caption{Comparative fault detection performance analysis on the Pronto Dataset under different fault types.}
\label{fig:pronto-result}
\end{figure}
\revtextrewrite{
We evaluate the performance of DyEdgeGAT on the Pronto dataset, considering three distinct fault types: air leakage, air blockage, and diverted flow. Figure~\ref{fig:pronto-result} shows the AUC scores for each fault type, as well as the average performance across all fault types. Baseline models exhibit varying performances for each fault type. However, DyEdgeGAT consistently demonstrates strong performance across all three fault types, highlighting its robust ability to detect relationship shifts for fault detection.
Air leakage is the easiest fault to detect, followed by air blockage and diverted flow. This observation is further supported by the performance of all models with relatively high AUC scores for air leakage but relatively low AUC scores for the other two fault types.

\textbf{Air Leakage.} Air leakage induces a cyclic behavior in the multiphase flow facility~\cite{stief2019pronto}, creating a distinct pattern that deviates significantly from the normal behavior. As shown in Figure~\ref{fig:pronto_dist}, the process variable PIC501 exceeds its normal range during air leakage. Therefore, detecting air leakage can be seen as a ``point anomaly'', making it easier to detect. Even though DyEdgeGAT does not perform the best on air leakage detection, it still demonstrates competitive performance.}

\revtext{\textbf{Air Blockage.} For this fault type, DyEdgeGAT outperforms all other baselines by a significant margin. Unlike the air leakage case, air blockage does not cause a reduction in pressure or a drop in the system. The flow remains continuous, making this fault type more challenging to detect.
In this class, FNN performs poorly, suggesting that modeling the static functional relationship alone is not sufficient. It is important to track the evolution of these relationships over time.}

\revtextrewrite{\textbf{Diverted Flow.}
Diverted Flow. This fault type is the most challenging for all baselines to detect, with all methods underperforming except for FNN and DyEdgeGAT. Graph-based models perform particularly poorly on this task.
Diverted flow induces noticeable changes in the flow regime within the multiphase flow facilities, leading to significant shifts in the functional relationships within the system. This explains why FNN performs well, as it can model these functional relationships.
The inability of other methods, even those that capture both temporal dynamics and spatial interdependencies, to detect this fault type suggests that the time series remain within their normal range and exhibit typical temporal patterns. This further emphasizes the need to model and capture changes in functional relationships within the system.
The significant drop in the performance of graph-based models on this task demonstrates the limitation of treating all variables as the same type of nodes in modeling relationships. This highlights the need to distinguish between variable types and incorporate operating condition contexts. 

In conclusion, DyEdgeGAT consistently outperforms baseline models in detecting a variety of faults, demonstrating its potential for broad applicability in complex industrial systems.}



%This could be attributed to the design of its anomaly score, which primarily focuses on the overall deviation of the system state, emphasizing particularly on shifts in relationships between signals. 
%In this scenario, the mean deviation arises due to changes in specific sensor values, such as that of pressure. Even though this fault introduces shifts in the relationships within the system, it primarily acts as a point anomaly rather than a collective anomaly.

%In the evaluation of the Pronto dataset, we consider three distinct fault types for detection. 
%Figure~\ref{fig:pronto-result} illustrates the AUC score for each fault type, as well as the average performance across all classes on the Pronto dataset. 
%Baseline models exhibit varying performances for each fault type, but notably, our proposed TimeGAT model consistently demonstrates strong performance across all fault types, highlighting its robust ability to detect relationship shifts in multivariate time series data.


%As shown in Fig.~\ref{fig:pronto_tsne}, \textit{diverted flow} is the most challenging fault to detect, while \textit{air leakage} is the easiest. 
%This observation is further supported by the performance of all models, which achieve relatively high AUC values for the \textit{air leakage} fault type but struggle to attain high scores for the \textit{diverted flow} fault type.


%For this fault type, all methods achieved relatively high AUC scores. 
%The air leakage fault induces a cyclic behavior in the multiphase flow facility~\cite{stief2019pronto}, creating a distinct pattern that deviates significantly from the normal behavior. 
%As shown in Fig.~\ref{fig:pronto_dist}, the process variable PIC501 exceeds its normal range during air leakage. Therefore, detecting this fault type can be seen as a \textit{point anomaly}, which is easier to detect.
%Even though not performing the best, TimeGAT still demonstrates competitive fault detection performance for this fault type.


%LSTM-AE, MTADGAT, and \revtext{TimeGAT} exhibit similar performance in terms of AUC, with \revtext{TimeGAT} leading by a small margin. However, \revtext{TimeGAT} achieves a higher F1 score compared to these methods, despite having a similar AUC score.
%As a result, all methods exhibit relatively low AUC scores for this fault type. 

%This fault type is the hardest on average for all baselines to detect. Except for FNN and TimeGAT, all methods underperform, especially for graph-based methods. 
%The diverted flow induces noticeable differences in the flow regime within the multiphase flow facilities, leading to significant shifts in the functional relationships within the system, this explains why FNN is performing well.

%The inability of all other methods, even those capturing both temporal dynamics and spatial interdependencies, to detect this fault type reveals that the time series remain within their normal range and exhibit typical temporal patterns. 
%This further emphasizes the necessity of modeling and capturing changes in functional relationships within the system.


%The significant drop in performance of graph-based methods in this class further shows the limitation of treating all variables as same type of nodes in modeling relationships.
%This further emphasizes the necessity of distinguishing variable types and incorporating operating condition contexts.

%In conclusion, \revtext{TimeGAT} consistently demonstrates robust and superior performance across all fault types, demonstrating its effectiveness in detecting a variety of faults. It showed exceptional capability in identifying faults involving shifts in functional relationships within the MTS data. This underscores \revtext{TimeGAT}'s potential for broad applicability in complex industrial systems.



To merge and revise the two parts while ensuring a smooth flow, the structure can be organized to first detail each fault type's specific detection challenges and DyEdgeGAT's performance, followed by a summary of the overall performance. Here's the revised text:

"\textbackslash{}subsubsection\{Fault Detection Performance Across Various Fault Types\}

We assessed DyEdgeGAT's performance on the Pronto dataset across three distinct fault types: air leakage, air blockage, and diverted flow. Figure\~\ref\{fig:pronto-result\} illustrates the AUC scores for each fault type and their average. While baseline models show varied performances for each fault type, DyEdgeGAT consistently exhibits strong performance across all, demonstrating its robustness in detecting relationship shifts.

\textbackslash{}textbf\{Air Leakage.\} Characterized by cyclic behavior in the multiphase flow facility, air leakage creates a noticeable deviation from normal patterns, making its detection relatively straightforward. DyEdgeGAT, though not the top performer in this category, still showcases competitive performance.

\textbackslash{}textbf\{Air Blockage.\} Here, DyEdgeGAT surpasses all baselines significantly. The continuous flow nature of air blockage, without obvious pressure drops, makes it a more complex fault to detect. The poor performance of FNN indicates the necessity of modeling evolving relationships over time for effective detection.

\textbackslash{}textbf\{Diverted Flow.\} This fault presents the most challenge, with only FNN and DyEdgeGAT performing adequately. Diverted flow leads to marked shifts in functional relationships, explaining FNN's success. The struggle of other models, including those adept in capturing temporal and spatial aspects, underscores the need for a nuanced approach in modeling variable types and incorporating operational contexts.

In summary, DyEdgeGAT's consistent outperformance across varied faults underscores its potential in complex industrial systems.

\textbackslash{}subsubsection\{Overall Performance Evaluation\}

As detailed in Tab.\~\ref\{tab:pronto\_results\}, DyEdgeGAT leads in AUC, F1, and F1\$^*\$ scores on the Pronto dataset and has the second-lowest detection delay. This points to its timely fault detection capability. Two key observations stand out:

\textbackslash{}textbf\{Importance of Functional Relationship Modeling\}: Models like FNN and AE, focusing on functional relationships, fare better than those emphasizing temporal dynamics. This suggests that changes in functional relationships are more critical than dynamic shifts in the Pronto dataset's context.

\textbackslash{}textbf\{Suboptimal Performance of GNN Models\}: GDN and GRELEN, the graph-based models, underperform, likely due to their inability to differentiate between system-dependent and independent variables. In the Pronto dataset, this distinction is vital, as faults don't affect system-independent variables in the same manner as system-dependent ones. The failure to make this distinction makes GNN methods prone to false fault detections under novel operating conditions."


==> chaps/bk/05-4-ablation_bk.tex <==
\subsection{RQ3: Ablation Study}
The goal of this ablation study is to evaluate the influence of each component of our proposed \revtext{TimeGAT} method on the overall performance. Through this analysis, we validate the methodological choices made in the design of \revtext{TimeGAT}.

Table~\ref{tab:all_ablation} reports the results of the ablation study on both synthetic and Pronto datasets. We consider four different ablation scenarios, indicated by the labels ``- w/o contr aug'', ``- w/o time enc'', ``- w/o att score'', and ``- w/o dyn edge'', which signify the removal of a specific component from the \revtext{TimeGAT} framework. Each label is explained as follows:

\begin{itemize}
\item \textbf{w/o contr aug}: The control parameter augmentation feature is excluded from \revtext{TimeGAT}. Without this component, the framework does not differentiate control parameters from other nodes, and they are treated as standard measurement nodes.
\item \textbf{w/o time enc}: This scenario omits the temporal encoding feature in \revtext{TimeGAT}, which could potentially weaken the model's ability to identify temporal dependencies.
\item \textbf{w/o att score}: In this setting, \revtext{TimeGAT} does not include the attention-based anomaly score, leading to uniform weights being assigned to all normalized node residuals. This absence may affect the effectiveness of anomaly detection.
\item \textbf{w/o dyn edge}: The dynamic edge construction component is removed. Instead, the attention mechanism from MTADGAT is used for feature graph construction, and the top-k mechanism from GDN is implemented to learn a sparse representation of the graph.
\end{itemize}

Examining \revtext{TimeGAT}'s performance under these scenarios allows us to evaluate the individual contributions of each component to the method's overall efficacy.

% pronto dataset
The findings for the Pronto dataset parallel those from the synthetic dataset. \revtext{TimeGAT} achieves the best performance, with the exclusion of the attention-based anomaly score resulting in a minor performance drop. The removal of the temporal encoding, control parameter augmentation, and dynamic edge construction, however, leads to a noticeable decrease in AUC and F1 scores, thus stressing the importance of these components.

% conclusion
In summary, this ablation study confirms that the attention-based anomaly score, temporal encoding, control parameter augmentation, and dynamic edge construction are all vital contributors to the superior performance of \revtext{TimeGAT}. Among these, the dynamic edge construction's absence appears to impact the AUC scores most significantly, emphasizing its role in modeling evolving relationships and intricate dependencies. Hence, this study substantiates the crucial importance of dynamic edge construction in improving the anomaly detection performance of our proposed \revtext{TimeGAT} method.

==> chaps/notations.tex <==
\section*{Nomenclature}
\addcontentsline{toc}{section}{Nomenclature}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$W = t-t_w + 1$}]
\item[Notion] Description
\item[$t \in \R$] current time.
\item[$t_w\in \R$] start time of the observation window.
\item[$\mathbf{X}^{t_w:t}\in\R^{N\times W}$] sliced measurement from time $t_w$ to $t$.
\item[$\mathbf{x}^{t_w:t}_{i} \in \mathbb{R}^{W}$] $i$-th measurement from time $t_w$ to $t$.
\item[${x}_{i}^{t}\in \R$] $i$-th sensor recording at time $t$.
\item[$N\in \N$] number of measurement variables.
\item[$\mathbf{U}^{t_w:t}\in\R^{N_u\times W}$] control variables from time $t_w$ to $t$.
\item[$\mathbf{u}^{t_w:t}_i \in \mathbb{R}^{W}$] $i$-th control variables from time $t$ to $t_w$.
\item[$N_u\in \N$] number of control variables.
\item[$W = t-t_w + 1$] length of the observation window.
\item[$\mathcal{V}=\{v_i\}$] set of nodes representing sensors.
\item[$\mathcal{E}=\{e_{ij}\}$] set of edges representing interactions between sensors.
\item[$\mathcal{G}=(\mathcal{V}, \mathcal{E})$] graph with nodes $\mathcal{V}$ and edges $\mathcal{E}$.
\item[$\delta t \in \R$] length of sliding window in dynamic edge construction.
\item[$\mathbf{A}^{t}\in \R^{|\mathcal{V}|\times|\mathcal{V}|}$] dynamic edge attributes at time $t$.
\item[$\mathbf{H}^{node}\in \R^{|\mathcal{V}|\times p}$] hidden node dynamic representation.
\item[$\mathbf{H}^{edge}\in \R^{|\mathcal{E}|\times p}$] hidden edge dynamic representation.
\item[$p\in \N$] dimension of node or edge attributes.
\item[$\mathbf{Z}\in \R^{|\mathcal{V}|\times p}$] hidden temporal graph representation.
\item[$\alpha_{ij}^t\in \R$] attention coefficient between node $i$ and $j$ at time $t$.
\end{IEEEdescription}


==> tabs/bk/all_ablation.tex <==
\begin{table}
\centering
\caption{Ablation study on synthetic and pronto datasets with 5 runs}
\begin{tabular}{llccc}
\toprule
 & & \textbf{AUC} $\uparrow$ & \textbf{F1}  $\uparrow$ & \textbf{Delay} $\downarrow$ \\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Synthetic}}} & \revtext{TimeGAT} & 0.874 ± 0.035 & 0.752 ± 0.045 & 14.3 ± 6.6 \\
& - w/o att score & 0.863 ± 0.036 & 0.762 ± 0.052 & 2.2 ± 6.5 \\
& - w/o time enc & 0.868 ± 0.027 & 0.694 ± 0.145 & 14.6 ± 6.9 \\
& - w/o contr aug & 0.831 ± 0.041 & 0.339 ± 0.165 & 72.2 ± 6.4 \\
& - w/o dyn edge & 0.803 ± 0.061 & 0.598 ± 0.234 & 17.0 ± 24.2 \\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Pronto}}} & \revtext{TimeGAT} & 0.766 ± 0.049 & 0.790 ± 0.011 & 36.5 ± 9.9 \\
& - w/o att score & 0.758 ± 0.046 & 0.787 ± 0.012 & 30.0 ± 0.0 \\
& - w/o time enc & 0.681 ± 0.090 & 0.786 ± 0.014 & 36.9 ± 12.2 \\
& - w/o contr aug & 0.731 ± 0.065 & 0.785 ± 0.015 & 48.5 ± 9.3 \\
& - w/o dyn edge & 0.677 ± 0.105 & 0.773 ± 0.043 & 44.1 ± 12.0 \\
\bottomrule
\end{tabular}
\label{tab:all_ablation}
\end{table}


==> tabs/bk/all_result.tex <==
% Please add the following required packages to your document preamble:

\begin{table}
\centering
\caption{Overall performance comparison on synthetic and pronto datasets with 5 runs. Best metric score is highlighted by bold.}
\begin{tabular}{llccc}
\toprule
 & & \textbf{AUC} $\uparrow$ & \textbf{F1}  $\uparrow$ & \textbf{Delay} $\downarrow$ \\
\midrule
\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Synthetic}}} & AE & 0.774 ± 0.025 & 0.584 ± 0.031 & 11.9 ± 2.4 \\
& FNN & 0.803 ± 0.018 & 0.572 ± 0.016 & 10.6 ± 0.7 \\
& LSTM & 0.814 ± 0.034 & 0.622 ± 0.001 & \textbf{10.0 ± 0.0}\\
& ENCDEC-AD & 0.832 ± 0.045 & 0.631 ± 0.015 & \textbf{10.0 ± 0.0} \\
& GDN & 0.795 ± 0.079 & \underline{0.667 ± 0.124} & 63.3 ± 14.5 \\
& MTADGAT & \underline{0.864 ± 0.018} & 0.621 ± 0.000 & \textbf{10.0 ± 0.0} \\
& \revtext{TimeGAT} & \textbf{0.874 ± 0.035} & \textbf{0.752 ± 0.045} & 24.3 ± 6.6 \\
\midrule
\multirow{7}{*}{\rotatebox[origin=c]{90}{\textbf{Pronto}}} & AE & 0.698 ± 0.019 & 0.562 ± 0.074 & 2928 ± 667 \\
& FNN & 0.646 ± 0.054 & 0.421 ± 0.020 & 3499 ± 71 \\
& LSTM & 0.672 ± 0.078 & \underline{0.765 ± 0.047} & \underline{38 ± 10} \\
& ENCDEC-AD & \underline{0.748 ± 0.034} & 0.569 ± 0.034 & 3399 ± 100 \\
& GDN & 0.498 ± 0.046 & 0.318 ± 0.013 & 4315 ± 559 \\
& MTADGAT & 0.696 ± 0.055 & 0.452 ± 0.056 & 3450 ± 1 \\
& \revtext{TimeGAT} & \textbf{0.766 ± 0.049} & \textbf{0.790 ± 0.011} & \textbf{37 ± 10} \\
\bottomrule
\end{tabular}
\label{tab:all_result}
\end{table}



==> tabs/bk/pronto_ablation_results.tex <==
\begin{table}
\centering
\caption{Ablation study on pronto dataset with 5 runs}
\label{tab:syn_ablation}
\begin{tabular}{llll}
\toprule
 & AUC & F1 & Delay \\
model &  &  &  \\
\midrule
\revtext{TimeGAT} & 0.747 ± 0.072 & 0.790 ± 0.011 & 31.0 ± 0.0 \\
- topol ad_score & 0.716 ± 0.081 & 0.769 ± 0.012 & 31.0 ± 0.0 \\
- time enc & 0.621 ± 0.138 & 0.726 ± 0.083 & 31.0 ± 0.0 \\
- contr aug & 0.648 ± 0.075 & 0.776 ± 0.038 & 31.0 ± 0.0 \\
- temp graph & 0.588 ± 0.140 & 0.639 ± 0.126 & 522.4 ± 972.8 \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/bk/pronto_agg_results.tex <==
\begin{table}
\centering
\caption{Performance comparison on pronto dataset with 5 runs. Best metric score is highlighted by bold}
\label{tab:pronto}
\begin{tabular}{llll}
\toprule
 & AUC & F1 & Delay \\
model &  &  &  \\
\midrule
AE & 0.691 ± 0.026 & 0.508 ± 0.051 & 3486 ± 15 \\
FNN & 0.633 ± 0.031 & 0.407 ± 0.009 & 3493 ± 0 \\
LSTM & 0.613 ± 0.104 & 0.749 ± 0.065 & \textbf{31 ± 0} \\
ENCDEC-AD & 0.701 ± 0.032 & 0.521 ± 0.048 & 3480 ± 1 \\
GDN & 0.423 ± 0.035 & 0.313 ± 0.014 & 4574 ± 457 \\
MTADGAT & 0.701 ± 0.040 & 0.516 ± 0.060 & 3479 ± 0 \\
\revtext{TimeGAT} & \textbf{0.747 ± 0.072} & \textbf{0.790 ± 0.011} & 31 ± 0 \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/bk/pronto_res_w_abl.tex <==
\begin{table}[tbhp]
\centering
\caption{Performance comparison on pronto dataset with 5 runs. The best metric score is highlighted in bold and the second best model in underscor}
\label{tab:pronto_agg_results}
\begin{tabular}{llccc}
\toprule
& & \textbf{AUC} $\uparrow$ & \textbf{F1}  $\uparrow$ & \textbf{Delay} $\downarrow$ \\
\midrule
\multicolumn{5}{l}{\textit{Only inter-dependencies}} \\

& FNN & 0.633 ± 0.031 & 0.407 ± 0.009 & 3493 ± 0 \\ 
& AE & 0.691 ± 0.026 & 0.508 ± 0.051 & 3486 ± 15 \\
\midrule
\multicolumn{5}{l}{\textit{Temporal and inter-dependencies}} \\
& LSTM & 0.613 ± 0.104 & \underline{0.749 ± 0.065} & \textbf{30 ± 0} \\
& ENCDEC-AD & \underline{0.701 ± 0.032} & 0.521 ± 0.048 & 3480 ± 1 \\
\midrule
\multicolumn{5}{l}{\textit{Temporal and inter-dependencies with graphs}} \\
& GDN & 0.423 ± 0.035 & 0.313 ± 0.014 & 4574 ± 457 \\
& MTADGAT & \underline{0.701 ± 0.040} & 0.516 ± 0.060 & 3479 ± 0 \\
\midrule
\multicolumn{5}{l}{\textit{Proposed method}} \\
& \revtext{TimeGAT} & \textbf{0.747 ± 0.072} & \textbf{0.790 ± 0.011} & \textbf{30 ± 0} \\
& - topol score & 0.753 ± 0.084 & 0.789 ± 0.012  & 30 ± 0 \\
& - time enc & 0.621 ± 0.138 & 0.726 ± 0.083 & 30 ± 0 \\
& - contr aug & 0.648 ± 0.075 & 0.776 ± 0.038 & 30 ± 0 \\
& - temp graph & 0.588 ± 0.140 & 0.639 ± 0.126 & 522.4 ± 972.8 \\
\bottomrule
\end{tabular}
\end{table}

==> tabs/bk/sy_res_w_abl_bk.tex <==
\begin{table}[htb]
\centering
\caption{Model Performance comparison on the synthetic dataset with 5 runs. The best metric score is highlighted in bold and the second best model in underscore}
\label{tab:syn_results}
\begin{tabular}{clccc}
\toprule
 & & \textbf{AUC} $\uparrow$ & \textbf{F1}  $\uparrow$ & \textbf{Delay} $\downarrow$ \\
\midrule
\multicolumn{5}{l}{\textit{Only inter-dependencies}} \\
 & FNN & 0.803 ± 0.018 & 0.572 ± 0.016 & 10.6 ± 0.7 \\
 & AE & 0.774 ± 0.025 & 0.584 ± 0.031 & 11.9 ± 2.4 \\
\midrule
\multicolumn{5}{l}{\textit{Temporal and inter-dependencies}} \\
 & LSTM & 0.814 ± 0.034 & 0.622 ± 0.001 & \textbf{10.0 ± 0.0} \\
 & ENCDEC-AD & 0.832 ± 0.045 & 0.631 ± 0.015 & \textbf{10.0 ± 0.0} \\
\midrule
\multicolumn{5}{l}{\textit{Temporal and inter-dependencies with graphs}} \\
 & GDN & 0.795 ± 0.079 & \underline{0.667 ± 0.124} & 29.3 ± 16.8 \\
 & MTADGAT & \underline{0.864 ± 0.018} & 0.621 ± 0.000 & \textbf{10.0 ± 0.0} \\ 
\midrule
\multicolumn{5}{l}{\textit{Proposed method}} \\
 & \revtext{TimeGAT} & \textbf{0.874 ± 0.035} & \textbf{0.752 ± 0.045} & 24.3 ± 6.6 \\
&- w/o att score & 0.863 ± 0.036 & 0.762 ± 0.052 & 12.2 ± 6.5 \\
&- w/o time enc & 0.868 ± 0.027 & 0.694 ± 0.145 & 14.6 ± 6.9 \\
&- w/o contr aug & 0.831 ± 0.041 & 0.339 ± 0.165 & 62.2 ± 6.4 \\
&- w/o temp graph & 0.803 ± 0.061 & 0.598 ± 0.234 & 17.0 ± 24.2 \\
\bottomrule
\end{tabular}
\end{table}

==> tabs/bk/syn_agg_results.tex <==
\begin{table}
\centering
\caption{Model Performance comparison on the synthetic dataset with 5 runs. The best metric score is highlighted in bold and the second best model in underscore}
\label{tab:syn_results}
\begin{tabular}{lccc}
\toprule
 & \textbf{AUC} $\uparrow$ & \textbf{F1}  $\uparrow$ & \textbf{Delay} $\downarrow$ \\
\midrule
AE & 0.774 ± 0.025 & 0.584 ± 0.031 & 11.9 ± 2.4 \\
FNN & 0.803 ± 0.018 & 0.572 ± 0.016 & 10.6 ± 0.7 \\
LSTM & 0.814 ± 0.034 & 0.622 ± 0.001 & \underline{\textbf{10.0 ± 0.0}} \\
ENCDEC-AD & 0.832 ± 0.045 & 0.631 ± 0.015 & 10.0 ± 0.0 \\
GDN & 0.795 ± 0.079 & \underline{0.667 ± 0.124} & 29.3 ± 16.8 \\
MTADGAT & \underline{0.864 ± 0.018} & 0.621 ± 0.000 & 10.0 ± 0.0 \\
\revtext{TimeGAT} & \textbf{0.874 ± 0.035} & \textbf{0.752 ± 0.045} & 24.3 ± 6.6 \\
\bottomrule
\end{tabular}
\end{table}



==> tabs/pronto/oc_ablation.tex <==
\begin{table}[htbp]
\caption{Different model configurations for ablation study of operating condition context augmentation.}
\centering
\begin{tabular}{ll}
\hline
\textbf{Acronym} & \textbf{Configuration} \\
\hline
MV & Only models the relationship between MV \\
MV+CV+EF & Models all variables in the same way \\
MV aug CV & Models MV as system-dependent and CV as system-independent variables \\
MV aug CV+EF & Models MV and EF as system-dependent variables and CV as system-independent variables \\
\hline
\end{tabular}
\label{your-label-here}
\end{table}


==> tabs/pronto/pronto_condition.tex <==
\begin{table}
\centering
\caption{Performance of the models on the Pronto dataset under novel operating conditions.}
\label{tab:pronto_condition}
\begin{tabular}{llllllllll}
\toprule
model & AE & FNN & LSTM & LSTM-AE & USAD & GDN & GRELEN & MTADGAT & TimeGAT \\
\midrule
\textbf{Ambiguity} & 0.56 ± 0.13 & 0.14 ± 0.01 & 0.81 ± 0.12 & 0.84 ± 0.10 & \textbf{0.90 ± 0.06} & 0.31 ± 0.06 & \underline{0.87 ± 0.06} & 0.08 ± 0.01 & 0.84 ± 0.11 \\
\textbf{FPR} & 0.03 ± 0.01 & 0.02 ± 0.01 & \underline{0.06 ± 0.03} & 0.05 ± 0.02 & 0.01 ± 0.01 & 0.00 ± 0.00 & 0.00 ± 0.00 & 0.01 ± 0.01 & \textbf{0.14 ± 0.12} \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/pronto/pronto_condition_all.tex <==
\begin{table}
\centering
\caption{Performance of the models on the Pronto dataset under novel operating conditions.}
\label{tab:pronto_condition}
\begin{tabular}{lll}
\toprule
 & \textbf{Ambiguity} & \textbf{FPR} \\
\midrule
AE & 0.11 ± 0.03 & 0.02 ± 0.01 \\
FNN & 0.14 ± 0.01 & 0.00 ± 0.01 \\
LSTM & 0.19 ± 0.08 & 0.00 ± 0.05 \\
LSTM-AE & 0.05 ± 0.01 & 0.00 ± 0.01 \\
USAD & \textbf{0.90 ± 0.06} & 0.06 ± 0.01 \\
GDN & 0.31 ± 0.06 & \underline{0.07 ± 0.00} \\ 
GRELEN & \underline{0.87 ± 0.06} & 0.01 ± 0.00 \\
MTADGAT & 0.08 ± 0.01 & 0.03 ± 0.01 \\ \midrule
TimeGAT & 0.84 ± 0.11 & \textbf{0.10 ± 0.12} \\
\bottomrule
\end{tabular}
\end{table}


==> tabs/pronto/pronto_res_all.tex <==
\begin{table*}[tbhp]
\centering
\caption{Performance comparison on pronto dataset with 5 runs. The best metric score is highlighted in bold and the second best model in underscor}
\label{tab:pronto_agg_results}
\begin{tabular}{lcccccc}
\toprule
 & \textbf{ROC AUC} $\uparrow$ & \textbf{PR AUC} $\uparrow$ & \textbf{F1} $\uparrow$ & \textbf{F1}$^*$ $\uparrow$ & \textbf{F1\textsubscript{PA\%50}} $\uparrow$ &  \textbf{Delay}$^*$ $\downarrow$ \\
\midrule
AE & 0.726 ± 0.039 & 0.779 ± 0.025 & 0.400 ± 0.016 & \underline{0.825 ± 0.023} & \underline{0.865 ± 0.027} & 905.1 ± 559.1 \\
FNN & \underline{0.745 ± 0.020} & 0.810 ± 0.011 & 0.634 ± 0.049 & 0.817 ± 0.007 & 0.857 ± 0.012 & 1644.1 ± 83.2 \\
LSTM & 0.603 ± 0.087 & 0.728 ± 0.047 & \underline{0.699 ± 0.109} & 0.796 ± 0.019 & 0.839 ± 0.047 & 510.9 ± 598.5 \\
LSTM-AE & 0.725 ± 0.037 & \underline{0.813 ± 0.019} & 0.607 ± 0.040 & 0.813 ± 0.006 & 0.848 ± 0.011 & 1952.4 ± 783.9 \\
USAD & 0.642 ± 0.017 & 0.740 ± 0.013 & 0.230 ± 0.015 & 0.801 ± 0.001 & 0.807 ± 0.003 & \textbf{47.1 ± 3.7} \\
GDN & 0.511 ± 0.062 & 0.674 ± 0.036 & 0.297 ± 0.042 & 0.783 ± 0.009 & 0.786 ± 0.011 & 1039.3 ± 838.7 \\
GRELEN & 0.458 ± 0.013 & 0.635 ± 0.010 & 0.252 ± 0.029 & 0.770 ± 0.000 & 0.770 ± 0.000 & 1892.7 ± 54.7 \\
MTADGAT & 0.680 ± 0.050 & 0.778 ± 0.025 & 0.402 ± 0.013 & 0.814 ± 0.008 & 0.852 ± 0.013 & 1521.7 ± 1.0 \\
TimeGAT & \textbf{0.801 ± 0.049} & \textbf{0.840 ± 0.043} & \textbf{0.826 ± 0.022} & \textbf{0.859 ± 0.017} & \textbf{0.895 ± 0.023} & \underline{60.9 ± 1.5} \\
\bottomrule
\end{tabular}
\end{table*}

==> tabs/toy/syn_res_all.tex <==
\begin{table*}[htbp]
\centering
\revtext{MENTION AVERAGE}
\caption{Model Performance comparison on the synthetic dataset with 5 runs. The best metric score is highlighted in bold and the second best model in underscore}
\label{tab:syn_res}
\begin{tabular}{lcccccc}
\toprule
 & \textbf{ROC AUC} $\uparrow$ & \textbf{PR AUC} $\uparrow$ & \textbf{F1} $\uparrow$ & \textbf{F1}$^*$ $\uparrow$ & \textbf{F1\textsubscript{PA\%50}} $\uparrow$ &  \textbf{Delay}$^*$ $\downarrow$ \\
\midrule
AE & 0.744 ± 0.028 & 0.646 ± 0.025 & 0.562 ± 0.028 & 0.631 ± 0.024 & 0.759 ± 0.048 & 30.0 ± 9.7 \\
FNN & 0.784 ± 0.019 & 0.698 ± 0.038 & 0.552 ± 0.009 & 0.666 ± 0.014 & 0.797 ± 0.040 & 21.7 ± 9.0 \\ \midrule
LSTM & 0.784 ± 0.037 & 0.778 ± 0.047 & 0.605 ± 0.003 & 0.702 ± 0.033 & 0.837 ± 0.070 & 23.3 ± 11.4 \\
LSTM-AE & 0.799 ± 0.052 & 0.746 ± 0.064 & 0.605 ± 0.002 & 0.722 ± 0.040 & 0.818 ± 0.057 & \textbf{9.2 ± 5.9} \\
USAD & 0.738 ± 0.000 & 0.746 ± 0.000 & 0.604 ± 0.000 & 0.673 ± 0.000 & 0.834 ± 0.000 & 39.7 ± 0.0 \\ \midrule
GDN & 0.777 ± 0.058 & 0.714 ± 0.070 & \underline{0.663 ± 0.074} & 0.718 ± 0.045 & 0.779 ± 0.056 & \underline{19.4 ± 10.6} \\
GRELEN & 0.673 ± 0.003 & 0.655 ± 0.003 & 0.421 ± 0.007 & 0.643 ± 0.003 & 0.696 ± 0.014 & 33.6 ± 3.2 \\
MTADGAT & \underline{0.806 ± 0.038} & \underline{0.788 ± 0.031} & 0.604 ± 0.000 & \underline{0.725 ± 0.036} & \underline{0.853 ± 0.045} & 25.2 ± 9.5 \\ \midrule
TimeGAT & \textbf{0.832 ± 0.040} & \textbf{0.806 ± 0.051} & \textbf{0.690 ± 0.076} & \textbf{0.750 ± 0.039} & \textbf{0.859 ± 0.060} & 21.4 ± 5.6 \\
\bottomrule
\end{tabular}
\end{table*}

% TODO: add evaluation of point anomaly (original implementation in the appendix)
